Expectation Entropy as a Password Strength Metric

The classical combinatorics-based password strength formula provides a result in tens of bits, whereas the NIST Entropy Estimation Suite give a result between 0 and 1 for Min-entropy. In this work, we present a newly developed metric -- Expectation entropy that can be applied to estimate the strength of any random or random-like password. Expectation entropy provides the strength of a password on the same scale as an entropy estimation tool. Having an 'Expectation entropy' of a certain value, for example, 0.4 means that an attacker has to exhaustively search at least 40\% of the total number of guesses to find the password.

==> sections/3_section.tex <==
\section{Min-entropy estimation methods}
In this section, we summarise some of the Min-entropy estimation methods used in the NIST entropy estimation tool.
The Most Common Value estimate finds the proportion  of the most common value in the input dataset, and then constructs a confidence interval for this proportion. The upper bound of the confidence interval is used to estimate the min-entropy per sample of the source.

The collision estimate, proposed by Hagerty and Draper \cite{hagerty2012entropy}, measures the mean number of samples to the first collision in the dataset, where collision means any repeated value. The goal of the method is to estimate the probability of the most-likely output value.

In a first-order Markov process, the next sample value depends only on the latest observed sample value; in an $n$th-order Markov process, the next sample value depends only on the previous $n$ observed values. Therefore, a Markov model can be used as a template for testing sources with dependencies. The Markov estimate provides a min-entropy estimate by measuring the dependencies between consecutive values from the input dataset.

The Compression Estimate is based on the Maurer Universal Statistical test \cite{maurer1992universal}. The estimate is computed by generating a dictionary of values, and then computing the average number of samples required to produce an output, based on the dictionary.

Tuple Estimate examines the frequency of $t$-tuples (pairs, triples, etc.) that appears in the input dataset and produces an estimate of the entropy per sample, based on the frequency of those tuples. 
